An open-source automated magnetic optical density meter for analysis of suspensions of magnetic cells and particles

We present a spectrophotometer (optical density meter) combined with electromagnets dedicated to the analysis of suspensions of magnetotactic bacteria. The instrument can also be applied to suspensions of other magnetic cells and magnetic particles. We have ensured that our system, called MagOD, can be easily reproduced by providing the source of the 3D prints for the housing, electronic designs, circuit board layouts, and microcontroller software. We compare the performance of our system to existing adapted commercial spectrophotometers. In addition, we demonstrate its use by analyzing the absorbance of magnetotactic bacteria as a function of their orientation with respect to the light path and their speed of reorientation after the field has been rotated by 90 degrees. We continuously monitored the development of a culture of magnetotactic bacteria over a period of five days, and measured the development of their velocity distribution over a period of one hour. Even though this dedicated spectrophotometer is relatively simple to construct and cost-effective, a range of magnetic field-dependent parameters can be extracted from suspensions of magnetotactic bacteria. Therefore, this instrument will help the magnetotactic research community to understand and apply this intriguing micro-organism.

==> sections/FutureApplications.tex <==
\subsection{Possible future applications}
The three experiments listed above are just some of the possibilities
offered by our novel MagOD system. Without additional modification,
we can imagine more experiments, which we report here to inspire
future work.

\subsubsection{Multi-color OD}
So far we have measured the transmission through MSR-1 cultures only
under green light. We notice however that the colour of cultures
changes as time passed by. We speculate that these colour changes may
be caused by an increase in bacteria size and/or formation of
magnetosomes. For long term analysis as in figure~\ref{fig:OD}, it may
therefore be usefull to measure at different wavelengths. In the MagOD
system, this can easily achieved by measuring iteratively with the
red, green and blue LED. Multiple wavelengths may be combined with the
addition of an indicator agent that changes its absorbance spectrum based on changes in conditions.

An example of such an indicator is Resazurin, which reacts to an increase
in oxygen concentration with a shift in the absorbance spectrum toward
the red. The ratio between the absorbance in the red and green
channels could therefore be a measure for the oxygen concentration in
the culture, using the blue channel for calibration.

\subsubsection{Modulated light intensity}
The intensity of the LEDs can be varied rapidly, as is illustated in
figure~\ref{fig:ModulatedSignal860}. One can use this modulation for
differential measurements to correct for intereference signals due to
changes in environmental light or cross-talk on the analog signal
wiring.

Modulation of the light intensity would also provide information on
the photosensitivity of the bacteria. One could for instance measure
the $C_\text{mag}$ in the red channel before and after a pulse with
intense blue light.

\subsubsection{Combined marathon and $C_\text{mag}$ }
We demonstrated $C_\text{mag}$ measurements on MSR-1 bacteria and
marathon tests on MC-1 bacteria. It is straightforward to combine the
marathon test with $C_\text{mag}$ measurements. The vertical field
($z$-direction) should than be switched between zero and for instance
a postive value, whereas the field along the light path
($x$-direction) should be switch between zero and alternatively
positive and negative values (So $(x,z)$={ (0,1), (1,0), (0,1),
  (-1,0), etc}). Such an experiment may reveal if the distribution in
velocity is related to a distribution in magnetosome strength as well.

\subsubsection{Sedimentation}
We often observe an initial increase of light transmission after
loading a sample with bacteria. We therefore usually wait until the
signal settles. However, there may be information we can extract. We
suspect the increase in transmission is caused by sedimentation of
debris, such as dead bacteria. If the dead bacteria have magnetosomes,
they will still rotate in the magnetic field. So a measurement of
$C_\text{mag}$ during sedimentation may provide additonal information
on the status of the culture.

Moreover, it is very simple to drive only one coil of the vertical
coil set. In this way one can generate field gradients that would pull
magnetic debris either up or down, thus decelerating or accelerating
the sedimentation.

\subsubsection{Suspensions of magnetic nanoparticles}
We often try the MagOD system with suspension of magnetic micro- and
nanoparticles. This works particularly well for magnetic
needles~\cite{Song2021} or magnetic discs~\cite{Loethman2018a}. In
principle, spherical particles should not show a change in
transmission under rotation of an external field. Magnetic particles
however have a tendency to form chains that align with the field (see
for instance the work by Yang Gao~\cite{Gao2013}). Angle and field
dependent transmission measurements in the MagOD could therefore
provide information on the dynamic interaction between
particles. Perhaps one can extend of the use of the MagOD beyond the
magnetotactic research community.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../MagOD"
%%% End:

